SegSplat: Feed-forward Gaussian Splatting and Open-Set Semantic Segmentation

We have introduced SegSplat, a novel framework designed to bridge the gap between rapid, feed-forward 3D reconstruction and rich, open-vocabulary semantic understanding. By constructing a compact semantic memory bank from multi-view 2D foundation model features and predicting discrete semantic indices alongside geometric and appearance attributes for each 3D Gaussian in a single pass, SegSplat efficiently imbues scenes with queryable semantics. Our experiments demonstrate that SegSplat achieves geometric fidelity comparable to state-of-the-art feed-forward 3D Gaussian Splatting methods while simultaneously enabling robust open-set semantic segmentation, crucially \textit{without} requiring any per-scene optimization for semantic feature integration. This work represents a significant step towards practical, on-the-fly generation of semantically aware 3D environments, vital for advancing robotic interaction, augmented reality, and other intelligent systems.

==> plots/3d_ovs_kmeans_plot.tex <==
\begin{figure}[htp]
  \centering
  \includegraphics[width=0.9\linewidth]{plots/3d_ovs/3d_ovs_kmeans_iou_comparison}
  \caption{
    We perform a search on the 3D-On the 3D-OVS dataset for the optimal $\lambda$ used to compute the number of clusters for each input (Section \ref{sec:experiments}).
    We observe that $\lambda=1.2$ yields the best performance while reducing the length of the feature encoding by $40 \%$ and producing IoU results nearly identical to those obtained with K-Means clustering disabled.
  }
  \label{fig:3d_ovs_kmeans_iou_comparison}
\end{figure}


==> plots/3d_ovs_langsplat_scene_comparison.tex <==
\begin{figure}[htp]
  \centering
  \subfloat[SegSplat]{
    \includegraphics[width=0.9\linewidth]{plots/3d_ovs/3d_ovs_segsplat_scene_comparison}
    \label{fig:segsplat}
  }\\[1mm]
  \subfloat[LangSplat]{
    \includegraphics[width=0.9\linewidth]{plots/3d_ovs/3d_ovs_langsplat_scene_comparison}
    \label{fig:langsplat}
  }
  \caption{
    Comparison of predicted and ground truth (GT) color and semantic maps for novel views rendered by SegSplat (a) and LangSplat (b) on the 3D-OVS dataset~\cite{liu2023weakly}.
    Semantic maps are visualized using PCA. Ground truth semantic features are obtained by applying SAM+CLIP to the corresponding GT novel view images.
    For LangSplat, we first decode the rendered semantic features using the learned autoencoder before applying PCA.
    Each group of four columns shows: GT RGB image, rendered RGB, GT semantics, and rendered semantics, repeated for two novel views.
    Our method (a) produces more accurate and less noisy semantic features compared to (b).
  }
  \label{fig:3d_ovs_side_by_side_scene_comparison}
  \vspace{-5mm}
\end{figure}


==> plots/re10k_segsplat_segmentation.tex <==
\begin{figure}[htp]
  \centering
  \includegraphics[width=0.25\linewidth]{plots/re10k/8adebbb68f2c3f84_segmentation}%
  \includegraphics[width=0.25\linewidth]{plots/re10k/34b0658a5c200cdf_segmentation}%
  \includegraphics[width=0.25\linewidth]{plots/re10k/e4f4574df7938f37_segmentation}%
  \includegraphics[width=0.25\linewidth]{plots/re10k/ed477bdf8582adff_segmentation}%
  \caption{A visualization of the masks produced by SegSplat on the RE10k dataset~\cite{realestate10k} using multiple text queries, as noted below each plot. We show results for four scenes and three different novel views in each scene.}
  \label{fig:re10k_segsplat_segmentations}
  \vspace{-5mm}
\end{figure}

